Efficient Contextformer: Spatio-Channel Window Attention for Fast Context Modeling in Learned Image Compression

Entropy estimation is essential for the performance of learned image compression. It has been demonstrated that a transformer-based entropy model is of critical importance for achieving a high compression ratio, however, at the expense of a significant computational effort. In this work, we introduce the Efficient Contextformer (eContextformer) - a computationally efficient transformer-based autoregressive context model for learned image compression. The eContextformer efficiently fuses the patch-wise, checkered, and channel-wise grouping techniques for parallel context modeling, and introduces a shifted window spatio-channel attention mechanism. We explore better training strategies and architectural designs and introduce additional complexity optimizations. During decoding, the proposed optimization techniques dynamically scale the attention span and cache the previous attention computations, drastically reducing the model and runtime complexity. Compared to the non-parallel approach, our proposal has ~145x lower model complexity and ~210x faster decoding speed, and achieves higher average bit savings on Kodak, CLIC2020, and Tecnick datasets. Additionally, the low complexity of our context model enables online rate-distortion algorithms, which further improve the compression performance. We achieve up to 17% bitrate savings over the intra coding of Versatile Video Coding (VVC) Test Model (VTM) 16.2 and surpass various learning-based compression models.

==> figures/figure1.tex <==
\begin{figure*}[!t]
\centering
% \captionsetup[subfigure]{labelformat=empty}

\subfloat[]{\includegraphics[page=9,width=0.165\textwidth,trim={2.25cm 11.4cm 2.5cm 2.25cm},clip]{figures/model5.pdf}}
\hfill
\subfloat[]{\includegraphics[page=10,width=0.165\textwidth,trim={2.25cm 11.4cm 2.5cm 2.25cm},clip]{figures/model5.pdf}}
\hfill
\subfloat[]{\includegraphics[page=11,width=0.165\textwidth,trim={2.25cm 11.4cm 2.5cm 2.25cm},clip]{figures/model5.pdf}}
\hfill
\subfloat[]{\includegraphics[page=12,width=0.165\textwidth,trim={2.25cm 11.4cm 2.5cm 2.25cm},clip]{figures/model5.pdf}}
\hfill
\subfloat[]{\includegraphics[page=13,width=0.165\textwidth,trim={2.25cm 11.4cm 2.5cm 2.25cm},clip]{figures/model5.pdf}}
\hfill
\subfloat[]{\includegraphics[page=14,width=0.165\textwidth,trim={2.25cm 11.4cm 2.5cm 2.25cm},clip]{figures/model5.pdf}}
\\
\subfloat[]{\input{figures/codingorder2.pgf}}\vspace{-2.1\baselineskip}
\subfloat[]{\includegraphics[page=15,width=0.165\textwidth,trim={2.25cm 8.8cm 2.5cm 4.8cm},clip]{figures/model5.pdf}}
\hfill
\subfloat[]{\includegraphics[page=16,width=0.165\textwidth,trim={2.25cm 11.4cm 2.5cm 2.25cm},clip]{figures/model5.pdf}}
\hfill
\subfloat[]{\includegraphics[page=17,width=0.165\textwidth,trim={2.25cm 11.4cm 2.5cm 2.25cm},clip]{figures/model5.pdf}}
\hfill
\subfloat[]{\includegraphics[page=18,width=0.165\textwidth,trim={2.25cm 11.4cm 2.5cm 2.25cm},clip]{figures/model5.pdf}}
\hfill
\subfloat[]{\includegraphics[page=19,width=0.165\textwidth,trim={2.25cm 11.4cm 2.5cm 2.25cm},clip]{figures/model5.pdf}}
\caption{Placeholder}
\label{fig_ctx_models}
\end{figure*}

==> tables/tab_perf2.tex <==
% \addtolength{\tabcolsep}{4pt}    
\begin{table}
    % \ra{1.3}
\newcolumntype{x}[1]{>{\centering\arraybackslash\hspace{0pt}}p{#1}}

    \addtolength{\tabcolsep}{-2pt}

	\centering
\begin{threeparttable}
	\caption{Performance of our model compared to various various learning-based codecs for various datasets}
	\label{tab_perf}
	\begin{tabular}{@{}lccccc@{}}
		\toprule
		& \multicolumn{5}{c}{BD-Rate [\%]$^a$} \\
	    \cmidrule(lr){2-6}
	    & & \multicolumn{3}{c}{CLIC2020~\cite{CLIC2020}}&\\
	    \cmidrule(lr){3-5}
		Method & \mc{Kodak~\cite{franzen1999kodak}} & -P && -M & \mc{Tecnick~\cite{asuni2014testimages}} \\
		\midrule
		eContextformer & $-10.9$ & $-11.5$ && $\phantom{1}\!\!-6.9$ & $-13.2$ \\
		\quad + oRDO         & $-14.7$ & $-13.6$ && $-10.4$ & $-17.1$ \\
		Contextformer~\cite{koyuncu2022contextformer} & $\phantom{1}\!\!-6.9$& $\phantom{1}\!\!-9.8$&& $\phantom{1}\!\!-5.8$& $-10.5$ \\
		\midrule
		Liu et al.~\cite{liu2023learned}(L)              & $-11.0$& &\textendash$^b$&& $-12.3$\\
		Liu et al.~\cite{liu2023learned}(S)              & $-11.0$& &\textendash$^b$&& $-12.3$\\
		He et al.~\cite{he2022elic}                   & $\phantom{1}\!\!-6.4$& &\textendash\phantom{$^b$}&& \textendash\\
		Wang et al.~\cite{wang2023evc}                & $\phantom{1}\!\!-1.1$ & &\textendash\phantom{$^b$}& & $\phantom{1}\!\!-0.7$ \\
		Fu et al.~\cite{fu2023asymmetric}             & $\phantom{1}\!\!-0.3$ & &\textendash\phantom{$^b$}& & \textendash\\
		Minnen\&Singh \cite{minnen2020channel}        & $\phantom{-1}1.7$&  &\textendash\phantom{$^b$}& & $\phantom{1}\!\!-2.2$ \\
		Cui et al.~\cite{cui2021asymmetric}           & $\phantom{-1}3.2$&  &{\textendash}\phantom{$^b$}& & \textendash \\
		Cheng et al.~\cite{cheng2020learned}       & $\phantom{-1}4.2$&  $\phantom{-1}5.9$& & $\phantom{-1}9.1$& $\phantom{-1}4.7$ \\
		He et al.~\cite{he2021checkerboard}           & $\phantom{-1}4.5$&  &{\textendash\phantom{$^b$}}& & $\phantom{-1}1.5$ \\
		Qian et al.~\cite{qian2021entroformer}        & $\phantom{-1}4.8$&  &{\textendash}$^b$& & \textendash \\
		Minnen et al.~\cite{minnen2018joint}          & $\phantom{-}15.6$& $\phantom{-}11.6$& &$\phantom{-}14.1$& $\phantom{-}15.4$ \\
		Yang\&Mandt~\cite{yang2023computationally}    & $\phantom{-}38.9$ & &\textendash\phantom{$^b$}&& $\phantom{-}45.7$ \\
		\quad + SGA~\cite{yang2020improving}            & $\phantom{-}24.9$ & &\textendash\phantom{$^b$}&&$\phantom{-}26.9$ \\
		BPG~\cite{bellard2015bpg}                     & $\phantom{-}30.3$& $\phantom{-}40.3$& &$\phantom{-}30.9$& $\phantom{-}29.5$ \\
		\bottomrule
	\end{tabular}
\begin{tablenotes}
\item[$^a$] Computed w.r.t. PSNR over VTM~16.2. Lower means higher bitrate savings.
\item[$^b$] Can not be computed due to out of memory (OOM)
\end{tablenotes}
\end{threeparttable}
\end{table}
